Discussion of "Nonparametric generalized fiducial inference for survival functions under censoring"

The following discussion is inspired by the paper Nonparametric generalized fiducial inference for survival functions under censoring by Cui and Hannig. The discussion consists of comments on the results, but also indicates it's importance more generally in the context of fiducial inference. A two page introduction to fiducial inference is given to provide a context.

==> def.tex <==
% def.tex
% 12/2-1991 (def.tex)
% 1998-06-15 15:08 (Fjerner IKKE AMS versjoner)
% 2004-01-15 19:52 (aoscm test)
% 2004-04-01 21:53 (elsart)

\usepackage{natbib}
\usepackage[utf8]{inputenc}
%\usepackage{url}

% \RequirePackage[OT1]{fontenc}
% \RequirePackage{amsthm,amsmath}
% %\RequirePackage[numbers]{natbib}
% \RequirePackage{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}

%\usepackage[a4paper]{geometry}
\usepackage[a4paper,includeheadfoot,margin=2.54cm]{geometry}


\usepackage{amsthm}
\usepackage{tikz-cd}



\newtheorem{Def}{Definition}
\newtheorem{prop}{Proposition}
\newtheorem{theo}{Theorem}



% My commands

\newcommand{\LossI}{L_{\textrm{I}}} % ...
\newcommand{\LossII}{L_{\textrm{II}}} % ... 

\newcommand{\lik}{=} % ... 

\newcommand{\darrow}{\overset{D}{\rightarrow}} % 

\newcommand{\halpha}{\hat{\alpha}} % 
\newcommand{\hbeta}{\hat{\beta}} % 

\newcommand{\ttau}{\tilde{\tau}} % 
\newcommand{\htau}{\hat{\tau}} % 
\newcommand{\tv}{\tilde{v}} % 
\newcommand{\hv}{\hat{v}} % 
\newcommand{\hw}{\hat{w}} % 
\newcommand{\tw}{\tilde{w}} % 
\newcommand{\htheta}{\hat{\theta}} % 
\newcommand{\ttheta}{\tilde{\theta}} % 

\newcommand{\ceps}{{\cal E}} % a sigma field
\newcommand{\cB}{{\cal B}} % a sigma field
\newcommand{\ca}{{\cal A}} % an Algebra
\newcommand{\cF}{{\cal F}} % an Algebra
\newcommand{\cE}{{\cal E}} % an Algebra
\newcommand{\cG}{{\cal G}} % an Algebra
\newcommand{\cT}{{\cal T}} % an Algebra

\newcommand{\barx}{\bar{x}} % 

\newcommand{\Si}{\operatorname{Si}} % The Sine integral function

\newcommand{\binorm}{\operatorname{binormal}}
\newcommand{\Cov}{\operatorname{Cov}}
%\newcommand{\Var}{\operatorname{Var}}


\newcommand{\pr}{\operatorname{\text{P}}} % Probability
\renewcommand{\Pr}{\operatorname{P}} % Probability
%\renewcommand{\Pr}{\operatorname{Pr}} % Probability
%\renewcommand{\Pr}{\operatorname{P}} % Probability
%\newcommand{\pr}{\operatorname{pr}} % Probability
%\newcommand{\pr}{\operatorname{\text{P}}} % Probability
\newcommand{\var}{\operatorname{var}} % Probability
\newcommand{\E}{{\operatorname{\text{E}}}} % Expectation
\newcommand{\Prob}{\mathord{\mbox{$P$}}} % Expectation

\newcommand{\setX}{{\text{\bf X}}} % A set X
\newcommand{\setT}{{\text{\bf T}}} % A set X
\newcommand{\setB}{{\text{\bf B}}} % A set X


\newcommand{\bset}{\Omega} % basic probability space
\newcommand{\bevents}{{\cal E}} % basic probability space

\newcommand{\bmu}{{\boldsymbol{\mu}}} % random variable
\newcommand{\bsigma}{{\boldsymbol{\sigma}}} % 
\newcommand{\bx}{{\boldsymbol{x}}} % 
\newcommand{\bv}{{\boldsymbol{v}}} % 
\newcommand{\br}{{\boldsymbol{r}}} % 

\newcommand{\bbchi}{{\boldsymbol{\chi}}} %
\newcommand{\bbp}{{\boldsymbol{p}}} % 
\newcommand{\bbs}{{\boldsymbol{s}}} % 
\newcommand{\bbu}{{\boldsymbol{u}}} % 
\newcommand{\bbv}{{\boldsymbol{v}}} % 
\newcommand{\bbw}{{\boldsymbol{w}}} % 
\newcommand{\bbT}{{\boldsymbol{T}}} % 
\newcommand{\bbpi}{{\boldsymbol{\pi}}} % 
\newcommand{\bbn}{{\boldsymbol{n}}} % 
\newcommand{\bbx}{{\boldsymbol{x}}} % 
\newcommand{\bby}{{\boldsymbol{y}}} % 
\newcommand{\bbt}{{\boldsymbol{t}}} % 
\newcommand{\bbr}{{\boldsymbol{r}}} % 
\newcommand{\bbz}{{\boldsymbol{z}}} % 
\newcommand{\bbtheta}{{\boldsymbol{\theta}}} % 
\newcommand{\bbsigma}{{\boldsymbol{\sigma}}} % 
\newcommand{\bbrho}{{\boldsymbol{\rho}}} % 

\newcommand{\half}{\frac{1}{2}} % half!

\newcommand{\HMean}[1]{\widetilde{#1}} % harmonic mean. Check ISO!

\newcommand{\m}{\operatorname{m}}
\newcommand{\mb}{\operatorname{M}}

\newcommand{\abs}[1]{\left| #1 \right|} 
%\newcommand{\Div}{\mathop{div}} 
%\newcommand{\curl}{\mathop{curl}} 
%\newcommand{\dlik}{\mathop{:=}\nolimits} 
%\newcommand{\E}{\operatorname{E}}
\newcommand{\Grad}{\mathop{\text{grad}}} 
%\newcommand{\into}{\mbox{$\: \rightarrow \:$}} 
%\renewcommand{\P}{\operatorname{P}}
\newcommand{\RealN}{{\mbox{$\mathbb R$}}} % Real numbers
\newcommand{\st}{\operatornamewithlimits{{\mid}}}
%\newcommand{\supp}{\mathop{\mbox{supp}}}
\newcommand{\Tr}{\mathop{\text{tr}}\nolimits} 
%\newcommand{\V}{\operatorname{Var}}

% Orddeling
% \hyphenation{ana-ly-sen}

\newcommand{\IG}{\mathop{IG}} % Inverse Gaussian
\newcommand{\Wald}{\mathop{Wald}} % Inverse Gaussian
\newcommand{\Normal}{\mathop{\text{N}}} % Normal, or Gaussian
\newcommand{\Uniform}{\mathop{Uniform}} % Uniform

\newcommand{\normvar}{\mathop{\bf N}}
\newcommand{\gamvar}{\mathop{\bf Gamma}}
\newcommand{\betavar}{\mathop{\bf Beta}}
\newcommand{\expvar}{\mathop{\bf Exp}}
\newcommand{\chitwovar}{\mathop{\bf \chi^2}}
\newcommand{\dirvar}{\mathop{\bf Dir}}
\newcommand{\univar}{\mathop{\bf U}}


% SI units
\newcommand{\SIm}{\text{m}} % meter
\newcommand{\SIcm}{\text{cm}} % centi meter
\newcommand{\SIs}{\text{s}} % seconds


% New commands
\newcommand{\hatt}{\hat{\theta}}
\newcommand{\Lloc}{L_{1,\text{loc}}}
%\newcommand{\E}{\mathop{\rm E}} % Expectation
%\newcommand{\E}{\mathop{\text{E}}} % Expectation
%\newcommand{\E}{\mathop{\mbox{$\Bbb E$}}} % Expectation


%\newcommand{\e}{\rm e} % 2.7...
\newcommand{\M}{\mathord{m}}
\newcommand{\s}{\mathord{s}}

\newcommand{\C}{\mathord{\cal C}}
\newcommand{\W}{\mathord{\cal W}}

\newcommand{\AW}{\mathord{{\hat{W}_A}}}
\newcommand{\AS}{\mathord{{S_A}}}
\newcommand{\AzDelta}{\mathord{{\Delta_{Az}}}}
\newcommand{\ADelta}{\mathord{{\Delta_{A}}}}

\newcommand{\BW}{\mathord{{\hat{W}_B}}}
\newcommand{\BtW}{\mathord{{\tilde{W}_B}}}
\newcommand{\BS}{\mathord{{S_B}}}
\newcommand{\BDelta}{\mathord{{\Delta_B}}}

%\DeclareMathOperator*{\Fhyp}{F}

\newcommand{\nc}{\newcommand}
\nc{\beqns}{\begin{eqnarray*}}
\nc{\eeqns}{\end{eqnarray*}}
\nc{\beqn}{\begin{eqnarray}}
\nc{\eeqn}{\end{eqnarray}}
\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\newcommand{\bes}{ \begin{equation} \begin{split} } %Nummerert slutt.
\newcommand{\ees}{ \end{split} \end{equation} } %Nummerert slutt.

\newcommand{\ii}{\mbox{\boldmath $\imath$}} % \sqrt{-1}
\newcommand{\beeq}[1]{\label{\knavn #1}} 
\newcommand{\be}[1]{\begin{equation}\label{eq#1}} 
\newcommand{\ee}{\end{equation}}%Nummerert slutt.
\newcommand{\eg}{{\it e g }}
\newcommand{\de}[1]{\stackrel{(\ref{\knavn #1})}{=}}
\newcommand{\id}{\mathop{id}}
\newcommand{\im}{\mathop{\mbox{Im}}\nolimits}
\newcommand{\Kg}{\mathord{kg}}
\newcommand{\li}[1]{{#1}\!-\!\lim\;}
\newcommand{\nn}{{nearest neighbor}}
\newcommand{\no}{\mathop{\mbox{\#}}\nolimits}
\newcommand{\Pa}{\mathord{Pa}}
\newcommand{\Hi}{ {\cal H} }
\newcommand{\gr}{\mathop{|}}
\newcommand{\hd}{\hat{\delta}}
\newcommand{\re}{\mathop{\mbox{Re}}\nolimits}
\newcommand{\Sc}{{S}chr{\"o}dinger\ }
\newcommand{\so}{{S}chr{\"o}dinger\ }
%\newcommand{\tr}{\mathop{\mbox{tr}}\nolimits}
%\newcommand{\Tr}{\mathop{\mbox{Tr}}\nolimits}

\newcommand{\alf}{Alf Taraldsen }                       
\newcommand{\bra}[1]{\left \langle #1 \right. |}
\newcommand{\COp}{{\cal C}} 
\newcommand{\der}[2]{ \frac{\partial #1}{\partial #2} }%Derivert.
\newcommand{\del}{\mathop{\triangle}}
\newcommand{\Div}{\mathop{\text{div}}}
\newcommand{\Ess}{\mathop{\mbox{Ess}}}
\newcommand{\etc}{{etc}} % et cetera, and the rest
\newcommand{\iid}{{i.i.d. }}
\newcommand{\Lin}{\mathop{\mbox{Lin}}}
\newcommand{\mto}{{\em mto}\ }
\newcommand{\pot}{{\cal P}}
\newcommand{\sgn}{\mathop{\mbox{sgn}}\nolimits} %Fortegnsfunksjon.      
\newcommand{\ess}{\mathop{\mbox{ess}}\nolimits}                 
\newcommand{\ket}[1]{\left. | #1 \right \rangle}
\newcommand{\Var}{\mathop{\mbox{Var}}\nolimits} % Variance

\newcommand{\curl}{\mathop{curl}\nolimits} 
%\newcommand{\dlik}{\stackrel{def}{=}}                          %Fire tegn.
\newcommand{\diam}{\mathop{\mbox{diam}}\nolimits} 
\newcommand{\dlik}{\mathop{=}\nolimits} % since := etc can be avoided ... 
\newcommand{\fpar}[1]{\left [ #1 \right ]}
\newcommand{\fsum}{\mathop{\dot{+}}} % 1992-07-28 17:38
% \newcommand{\Grad}{\mathop{\mbox{\bf grad}}}
%\newcommand{\half}{\frac{1}{2}} 
\newcommand{\IntN}{{\mbox{$\bf Z$}}} % Integers
\newcommand{\into}{\mbox{$\: \rightarrow \:$}} 
\newcommand{\konj}[1]{\overline{#1}}
\newcommand{\kpar}[1]{\left \{#1\right \}}
\newcommand{\likd}{\mathop{=:}\nolimits} 
\newcommand{\lims}{\mathop{\overline{\lim}\;}}
\newcommand{\limi}{\mathop{\underline{\lim}\;}}
\newcommand{\llim}{\mathop{l\!-\!\lim\;}}
\newcommand{\lsum}{\mathop{\hat{+}}} % 1992-07-28 17:08
\newcommand{\maxm}{m_{\text{max}}}
\newcommand{\mean}[1]{\left \langle#1 \right \rangle }
\newcommand{\NatN}{{\mbox{$\Bbb N$}}} % Natural numbers: 1, 2, ...
\newcommand{\norm}[1]{\left \| #1\right\|}
\newcommand{\nlim}{\mathop{n\!-\!\lim\;}}
\newcommand{\plim}{\mathop{p\!-\!\lim\;}}
\newcommand{\refl}[1]{(\ref{\knavn #1})} 
\newcommand{\refp}[1]{\refl{#1} p\aa\ side \pageref{#1}}  %Anngir og side.
\newcommand{\rpar}[1]{\left (#1\right )}                
\newcommand{\RatN}{{\mbox{$\Bbb Q$}}} % Rational numbers
\newcommand{\Real}{{\mbox{$\Bbb R$}}} % Real numbers\mbox{$\Bbb C$}
\newcommand{\slim}{\mathop{s\!-\!\lim\;}}
\newcommand{\supp}{\mathop{\mbox{supp}}}
\newcommand{\ulim}{\mathop{u\!-\!\lim\;}}
\newcommand{\vlim}{\mathop{v\!-\!\lim\;}}
\newcommand{\wlim}{\mathop{w\!-\!\lim\;}}
\newcommand{\Vlim}{\mathop{V\!-\!\lim\;}}
\newcommand{\Didx}[1]{\index{#1}}

%\newcommand{\CompN}{{\mbox{$\bf C$}}}
\newcommand{\CompN}{{\mbox{$\Bbb C$}}}                           %Fem
\newcommand{\QuartN}{{\mbox{$\Bbb H$}}}
\newcommand{\OctN}{{\mbox{$\Bbb O$}}}  
\newcommand{\compl}{\mathop{\sim}}
\newcommand{\gtdef}[1]{{\em #1}}
\newcommand{\imply}{\Rightarrow}
\newcommand{\lkpar}[1]{\left\{ \begin{array}{ll} #1 \end{array}\right.}
\newcommand{\Lclim}{\mathop{L_c\!-\!\lim\;}}
\newcommand{\Lilim}{\mathop{L_i\!-\!\lim\;}}
\newcommand{\Lmlim}{\mathop{L_m\!-\!\lim\;}}
\newcommand{\pplus}{\dot{+}}
\newcommand{\Uclim}{\mathop{U_c\!-\!\lim\;}}
\newcommand{\Umlim}{\mathop{U_m\!-\!\lim\;}}
\newcommand{\uclim}{\mathop{\tilde{u}\!-\!\lim\;}}
\newcommand{\uthev}[1]{{\it #1}}
\newcommand{\Vclim}{\mathop{\tilde{V}\!-\!\lim\;}}
\newcommand{\vclim}{\mathop{\tilde{v}\!-\!\lim\;}}
%\newcommand{\RealN}{{\mbox{$\Bbb R$}}} % Real numbers
\newcommand{\csigma}{{\tilde{\sigma}}}

\newcommand{\braket}[2]{\left \langle #1 | #2 \right \rangle }
\newcommand{\figtxt}{\footnotesize} % Size on figure texts
\newcommand{\hanche}{Harald \mbox{Hanche-Olsen} }
\newcommand{\holden}{Helge Holden }
\newcommand{\sarrow}{\stackrel{s}{\rightarrow}}
%\newcommand{\setdif}{\bigtriangleup}
\newcommand{\warrow}{\stackrel{w}{\rightarrow}}

\newcommand{\Complex}{\mbox{$\bf C$}}
\newcommand{\martens}{Henrik Martens }
\newcommand{\svektor}[2]{\fpar{\begin{array}{cc} #1\\#2 \end{array} }} %Vektor.

\newcommand{\rsvektor}[2]{\left .\begin{array}{ccc}
&\multicolumn{2}{c}{#1}\\
&\multicolumn{2}{c}{#2}\end{array} \right ]} %Stor matrise,
\newcommand{\lsvektor}[2]{\left [\begin{array}{c} #1,\\#2,\end{array}\right .} %Stor matrise.


